GPU-Accelerated Batch-Dynamic Subgraph Matching

Subgraph matching has garnered increasing attention for its diverse real-world applications. Given the dynamic nature of real-world graphs, addressing evolving scenarios without incurring prohibitive overheads has been a focus of research. However, existing approaches for dynamic subgraph matching often proceed serially, retrieving incremental matches for each updated edge individually. This approach falls short when handling batch data updates, leading to a decrease in system throughput. Leveraging the parallel processing power of GPUs, which can execute a massive number of cores simultaneously, has been widely recognized for performance acceleration in various domains. Surprisingly, systematic exploration of subgraph matching in the context of batch-dynamic graphs, particularly on a GPU platform, remains untouched. In this paper, we bridge this gap by introducing an efficient framework, GAMMA (GPU-Accelerated Batch-Dynamic Subgraph Matching). Our approach features a DFS-based warp-centric batch-dynamic subgraph matching algorithm. To ensure load balance in the DFS-based search, we propose warp-level work stealing via shared memory. Additionally, we introduce coalesced search to reduce redundant computations. Comprehensive experiments demonstrate the superior performance of GAMMA. Compared to state-of-the-art algorithms, GAMMA showcases a performance improvement up to hundreds of times.

==> Definitions.tex <==
\begin{table}

\centering
\small
\caption{Symbols and Descriptions}
\vspace{-2mm}
\label{tab:symbol}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{1.3cm}|p{6.9cm}|}
\hline
\textbf{Notation} & \textbf{Description} \\
\hline
$V$, $E$, $X$                  & The node, edge, and node feature sets                                                    \\ \hline
$v_i$, $e_{ij}$, $x_i$      & The $i$-th node and its incident edge and feature                                                     \\ \hline
$\mathcal{A}$, $\mathcal{R}$                   & The node and edge type sets                                           \\ \hline
$\mathbf{A}$, $\tilde{\mathbf{A}}$             & The adjacent matrix and its counterpart with self-loops               \\ \hline
$\tilde{\mathbf{D}}$               & The degree matrix w.r.t. $\tilde{\mathbf{A}}$                                       \\ \hline
$\phi$, $\psi$                  & The node and edge type mapping functions                              \\ \hline
$T_G$                  & The network schema                                                    \\ \hline
$\mathbf{X}$, $\mathbf{H}$, $\mathbf{Z}$                 & Node features, hidden states and node embeddings                  \\ \hline
$\hat{\mathbf{X}}$, $\hat{\mathbf{A}}$ & Reconstructed node features and adjacent matrix \\ \hline
$h_i$, $z_i$              & \multicolumn{1}{m{7cm}|}{The hidden states and node embeddings w.r.t. to node $v_i$} \\ \hline
$\mathbf{W}$, $\hat{\mathbf{W}}$ & Learnable weight matrices                                         \\ \hline
$\mathbf{b}$, $\hat{\mathbf{b}}$ & Learnable bais                                                    \\ \hline
$\{y_i\}$                & The cluster set                                                   \\ \hline
$\{u_j\}$                & The learned cluster centroids                                     \\ \hline
$\lambda$, $\gamma$, $\beta$      & The balancing coefficients                                            \\ \hline

\end{tabular}
\vspace{-4mm}
\end{table}

\section{Problem Definition}
\label{sec:definitions}

In this section, we first introduce some basic concepts, and then we formulate the studied problem. The frequently used notations are summarized in Table~\ref{tab:symbol}.


\begin{definition}
\label{def:hin}
    {\bf (Heterogeneous Information Network, HIN}. A HIN is denoted  as $G=(V,E,X,\phi, \psi)$, where (i) $V$ is the set of nodes; (ii) $E$ is the set of edges; (iii) $X$ is the set of features assigned to each node in the network; (iv) $\phi: V \rightarrow \mathcal{A}$ is a node type mapping function that maps each node in $V$ to a type in $\mathcal{A}$; and (v) $\psi: E \rightarrow \mathcal{R}$ is an edge type mapping function that maps each edge in $E$ to a relation type in $\mathcal{R}$. Here, $\mathcal{A}$ and $\mathcal{R}$ denote the sets of node types and edge types, respectively, and $\left| \mathcal{A}\right| + \left| \mathcal{R}\right| > 2$. In addition, for each $x_i \in X$ denoting the feature of vertex $v_i$,  $x_i \in \mathbb{R}^d$, and $d$ is the dimension of a feature vector. 
\end{definition}

\begin{definition}
\label{def:schema}
    {\bf (Network Schema}. The network schema of a HIN $G=(V,E,X,\phi, \psi)$, denoted as $T_{G}=(\mathcal{A}, \mathcal{R})$, is a meta template or schematic graph representing the relation between different types of nodes in $G$, where $\mathcal{A}$ is the node type set and $\mathcal{R}$ is the relation type set.
\end{definition}

Fig.~\ref{fig:illustration}(a) depicts a HIN of a bibliographic graph, which includes four node types (i.e., $\mathcal{A}$ = \{P, A, C, T\}) and three edge types (i.e., the set $\mathcal{R}$ = \{P-A, P-C, P-T\}). The network schema of this HIN is shown in Fig.~\ref{fig:illustration}(d). The network schema reveals that a paper, associated with certain terms, is written by an author and published in a conference.

\begin{definition}
\label{def:metapath}
    {\bf (Meta-path)}. A meta-path $\mathcal{P}$ of a network schema $T_{G}=(\mathcal{A}, \mathcal{R})$, denoted in the form of $A_{1} \stackrel{R_{1}}{\longrightarrow} A_{2} \stackrel{R_{2}}{\longrightarrow} \ldots \stackrel{R_{l}}{\longrightarrow} A_{l+1}$ (abbr. $A_{1}-A_{2}- \ldots- A_{l+1}$), is a path that represents a composition of relation $R=R_{1} \circ R_{2} \circ \ldots \circ R_{l}$ between type $A_{1}$ and $A_{l+1}$, where $\circ$ is the composition operator on relations.
\end{definition}


Take Fig.~\ref{fig:illustration} as an example again, where Fig.~\ref{fig:illustration}(b) shows two meta-paths P-A-P and P-C-P. Fig.~\ref{fig:illustration}(c) gives the meta-path instances (i.e., homogeneous networks) transformed via two meta-paths respectively. For instance, given the meta-path P-A-P, $P_{2}$ and $P_{3}$ are neighbors of $P_{1}$; while given the meta-path P-C-P, $P_{1}$ only has one neighbor $P_{2}$.
Based on the above concepts, we formally define the studied problem in this paper.

%\begin{definition}
%\label{def:problem}
%{\bf (HIN Co-Clustering)}. Given an attributed heterogeneous information network $G=(V,E,X,\phi, \psi)$, the AHIN co-clustering on $G$ aims to divide the multiple types of nodes in $G$ into $k$ disjoint groups $\{g_1, ..., g_k\}$, such that the nodes within the same group are typically close to each other considering the topological structure proximity and the attribute similarity.
% \end{definition}

\begin{definition}
\label{def:problem}
    {\bf (HIN Clustering)}. Given a HIN $G=(V,E,X,\phi, \psi)$, the HIN clustering on $G$ aims to divide the node set of the same type into $k$ disjoint groups $\{g_1, ..., g_k\}$, such that the nodes within the same group are typically close to each other. Here, close to each other refers: (i) similar to each other considering the topological structure regarding of HIN, i.e., under certain meta-path constraints, and (ii) similar to each other considering the features of nodes.
\end{definition}

Definition~\ref{def:problem} only clusters one type of nodes. Our problem also supports {\bf Co-clustering}, i.e., we clustering multiple types of nodes simultaneously. More specifically, we perform clustering for two different types of nodes at the same time.



